Harnessing Business and Media Insights with Large Language Models

This paper introduces Fortune Analytics Language Model (FALM). FALM empowers users with direct access to comprehensive business analysis, including market trends, company performance metrics, and expert insights. Unlike generic LLMs, FALM leverages a curated knowledge base built from professional journalism, enabling it to deliver precise and in-depth answers to intricate business questions. Users can further leverage natural language queries to directly visualize financial data, generating insightful charts and graphs to understand trends across diverse business sectors clearly. FALM fosters user trust and ensures output accuracy through three novel methods: 1) Time-aware reasoning guarantees accurate event registration and prioritizes recent updates. 2) Thematic trend analysis explicitly examines topic evolution over time, providing insights into emerging business landscapes. 3) Content referencing and task decomposition enhance answer fidelity and data visualization accuracy. We conduct both automated and human evaluations, demonstrating FALM's significant performance improvements over baseline methods while prioritizing responsible AI practices. These benchmarks establish FALM as a cutting-edge LLM in the business and media domains, with exceptional accuracy and trustworthiness.

==> sections/evaluation.tex <==
\section{Evaluation}
In this section, we conduct a comprehensive analysis of the model's performance across various aspects: business-centric question answering, data visualization, content referencing, and responsible AI. We employ two evaluation methodologies: comparative evaluation and independent evaluation.

\paragraph{Comparative Evaluation} This evaluation involves comparing responses generated by different models and evaluating their corresponding win rates. Comparative evaluation is beneficial for tasks where there is no golden ground truth, such as answering the question ``\emph{Can you tell me more about recent news on inflation?}'' Human judgment plays a crucial role in this process as human evaluators compare answers from various models based on fluency, accuracy, and relevance \citep{ribeiro2020beyond}. To complement human evaluation, we use LLM-based evaluation tools such as Prometheus \citep{kim2024prometheus}, which leverage language models to assess text quality. This approach allows for systematic evaluations at scale \citep{celikyilmaz2020evaluation,hackl2023gpt}. However, a drawback is that LLM-based tools may favor model responses similar to their training corpus or style \citep{dubois2024length}. Our evaluation pipeline integrates both LLM-based and human evaluators for a balanced approach between scalability and human alignment~\citep{gehrmann2021gem}.

\paragraph{Independent Evaluation} In this method, we analyze the response from one model and evaluate its performance based on predefined metrics or ground truths. For instance, in Metric QA, we will assess the exact match of requested metrics. In data visualization, we will determine if the output chart aligns with user queries. Independent evaluation can also be categorized into three primary categories: statistical measures, human-defined rubrics, and LLM-based or human evaluations. Statistical measures such as BLEU \citep{papineni2002bleu}, ROUGE \citep{lin2004rouge}, and METEOR \citep{banerjee2005meteor} are commonly used to assess the similarity between generated text and reference text. Similarly, LLM-based evaluation and human evaluators with customized rubrics (i.e., fluency, coherence, relevance, and factual accuracy) \citep{ribeiro2020beyond,lin-etal-2022-truthfulqa} are also widely adopted in independent evaluations. Human judgment remains crucial for assessing text quality based on factors such as fluency, accuracy, relevance, and truthfulness.



\input{fortune/sections/evaluation/patha}
\input{fortune/sections/evaluation/pathb}


